You May Not Need Ratio Clipping in PPO

Proximal Policy Optimization (PPO) methods learn a policy by iteratively performing multiple mini-batch optimization epochs of a surrogate objective with one set of sampled data. Ratio clipping PPO is a popular variant that clips the probability ratios between the target policy and the policy used to collect samples. Ratio clipping yields a pessimistic estimate of the original surrogate objective, and has been shown to be crucial for strong performance. We show in this paper that such ratio clipping may not be a good option as it can fail to effectively bound the ratios. Instead, one can directly optimize the original surrogate objective for multiple epochs; the key is to find a proper condition to early stop the optimization epoch in each iteration. Our theoretical analysis sheds light on how to determine when to stop the optimization epoch, and call the resulting algorithm Early Stopping Policy Optimization (ESPO). We compare ESPO with PPO across many continuous control tasks and show that ESPO significantly outperforms PPO. Furthermore, we show that ESPO can be easily scaled up to distributed training with many workers, delivering strong performance as well.

==> Makefile <==
# This script is initially borrowed from Wendelin Boehmer

NAME=main
APPENDIX=12
CONF=iclr2021

all: 
	pdflatex $(NAME).tex
	make bib
	pdflatex $(NAME).tex
	pdflatex $(NAME).tex
	make clean
	#make submit

bib: 
	if [ -e $(NAME).aux ] ; \
	then \
		echo COMPILE BIBTEX; \
		bibtex $(NAME).aux; \
	else \
		echo NO REFERENCES TO COMPILE; \
	fi;


submit:
	echo SPLIT PDF IN SUBMISSION AND APPENDIX
	$(eval END=$(shell echo $$(($(APPENDIX)-1))))
	pdftk $(NAME).pdf cat 1-$(END) output $(CONF)_submission.pdf
	pdftk $(NAME).pdf cat $(APPENDIX)-end output $(CONF)_supplementary.pdf

clean:
	rm -f $(NAME).aux $(NAME).bbl $(NAME).log $(NAME).out $(NAME).toc $(NAME).blg $(NAME).dvi $(NAME).ps $(NAME).nav $(NAME).snm $(NAME).vrb shortcuts.aux $(NAME).acn $(NAME).acr $(NAME).alg $(NAME).glg $(NAME).glo $(NAME).gls $(NAME).ist


